Deep Graph Random Process for Relational-Thinking-Based Speech Recognition

Lying at the core of human intelligence, relational thinking is characterized by initially relying on innumerable unconscious percepts pertaining to relations between new sensory signals and prior knowledge, consequently becoming a recognizable concept or object through coupling and transformation of these percepts. Such mental processes are difficult to model in real-world problems such as in conversational automatic speech recognition (ASR), as the percepts (if they are modelled as graphs indicating relationships among utterances) are supposed to be innumerable and not directly observable. In this paper, we present a Bayesian nonparametric deep learning method called deep graph random process (DGP) that can generate an infinite number of probabilistic graphs representing percepts. We further provide a closed-form solution for coupling and transformation of these percept graphs for acoustic modeling. Our approach is able to successfully infer relations among utterances without using any relational data during training. Experimental evaluations on ASR tasks including CHiME-2 and CHiME-5 demonstrate the effectiveness and benefits of our method.

==> Table/tbl-models.tex <==
\begin{table}
	\caption{WER (\%) on evaluation sets of CHiME-2, WSJ0 and WSJ0\&1.}
	\label{tbl-models}
	\centering
	\begin{tabular}{llll}
		\toprule
		
		{\sf Model}  & CHiME-2 & WSJ0 & WSJ0\&1  \\ 
		\midrule
		LSTM       & 26.1                           & 2.8        & 7.4              \\ 
		SRU        & 26.2                           & 2.8        & 7.5              \\ 
		Quasi-RNN  & 26.1                           & 2.8        & 7.4              \\ 
		RPPU       & 24.4                           & 2.5        & 6.9             \\ 
		\bottomrule
	\end{tabular}
\end{table}











==> Table/tbl-similarity.tex <==
\begin{table}
\caption{Similarity with the ground-truth phoneme-level alignment for our baseline and  estimated alignment using RPP on development set of CHiME-2 }
\label{tbl-simi}
  \centering
  \begin{tabular}{lll}
    \toprule

Alignment type                 & Similarity(\%) \\
    \midrule
Baseline alignment    & 55.5           \\ 
Estimated alignment using RPP & \textbf{64.7}           \\ 
    \bottomrule
  \end{tabular}
\end{table}
